Deep Learning for Generalised Planning with Background Knowledge

Automated planning is a form of declarative problem solving which has recently drawn attention from the machine learning (ML) community. ML has been applied to planning either as a way to test `reasoning capabilities' of architectures, or more pragmatically in an attempt to scale up solvers with learned domain knowledge. In practice, planning problems are easy to solve but hard to optimise. However, ML approaches still struggle to solve many problems that are often easy for both humans and classical planners. In this paper, we thus propose a new ML approach that allows users to specify background knowledge (BK) through Datalog rules to guide both the learning and planning processes in an integrated fashion. By incorporating BK, our approach bypasses the need to relearn how to solve problems from scratch and instead focuses the learning on plan quality optimisation. Experiments with BK demonstrate that our method successfully scales and learns to plan efficiently with high quality solutions from small training data generated in under 5 seconds.

==> figures/intro_figure_v1.tex <==
\begin{figure}[t]
	\centering
	\resizebox*{\columnwidth}{!}{
		\begin{tikzpicture}[scale=.8]
			\node[text width=1.5cm, align=center, draw, rectangle, rounded corners] (program) {$\delta$-Datalog\\ Program};
			\node[text width=1.5cm, align=center, above left=-0.2cm and 0.9cm of program, draw, rectangle, rounded corners] (KB) {background\\ knowledge};
			\node[text width=1.5cm, align=center, below left=-0.2cm and 0.9cm of program, draw, rectangle, rounded corners] (GNN) {message\\ passing};
			
			\node[right=1.5cm of program, draw, dashed, circle, minimum size=1.2cm] (train) {Train};
			\node[text width=1.2cm, align=center, above=0.9cm of train, draw, rectangle, rounded corners] (data) {data};
			
			\node[right=1.9cm of train, draw, dashed, circle, minimum size=1.2cm] (test) {Test};
			\node[text width=1.2cm, align=center, above=0.9cm of test, draw, rectangle, rounded corners] (instance) {problem};
			\node[text width=1.2cm, align=center, below=0.4cm of test, draw, rectangle, rounded corners] (search) {GBFS};
			
			
			\draw[-latex] (KB) -- node[above] {rules} (program);
			\draw[-latex] (GNN) -- node[below] {rules} (program);
			\draw[-latex] (program) -- node[above] {initial} node[below] {policy} (train);
			\draw[-latex] (data) -- node[left] {optimal} node[right] {actions} (train);
			\draw[-latex, dashed] (train) -- node[below, near start] {$\bm\theta$} node[below, near end] {$\bm\theta^{*}$} node[above] {parameters} (test);
			\draw[-latex] (instance) -- node[left] {initial}  node[right]{state} (test);
			\draw[-latex] (search) -- (test);
			\coordinate[right=1.2cm of test] (out);
			\draw[-latex] (test) -- node[above] {quality} node[below] {plan} (out);
			
	\end{tikzpicture}}
	\caption{Outline of the proposed approach}
	\label{fig:intro}
\end{figure}

==> sections/checklist.tex <==
\newpage
\section*{Reproducibility Checklist}

This paper:

\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced [yes]
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results [yes]
    \item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper [yes]
\end{itemize}

\noindent
% GS: I would personally put yeses here except for the proofs... I don't believe it is meant in a too strict manner... but up to you
% DC: It's hard to say since we don't have any concrete theorems and just formalising definitions and assumptions. I think I'm happy to put some yeses based on the formalisations
Does this paper make theoretical contributions? [yes] Theoretical contributions are in the form of formalising the problem setup and properties of such problems and their solutions. They are not theorem statements, hence all subquestions are answered NA.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. [NA]
    \item All novel claims are stated formally (e.g., in theorem statements). [NA]
    \item Proofs of all novel claims are included. [NA]
    \item Proof sketches or intuitions are given for complex and/or novel results. [NA]
    \item Appropriate citations to theoretical tools used are given. [NA]
    \item All theoretical claims are demonstrated empirically to hold. [NA]
    \item All experimental code used to eliminate or disprove claims is included. [NA]
\end{itemize}

\noindent
Does this paper rely on one or more datasets? [yes]
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets [yes]
    \item All novel datasets introduced in this paper are included in a data appendix. [NA]
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. [NA]
    \item All datasets drawn from the existing literature (potentially including authors' own previously published work) are accompanied by appropriate citations. [yes]
    \item All datasets drawn from the existing literature (potentially including authors' own previously published work) are publicly available. [yes]
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. [NA]
\end{itemize}

\noindent
Does this paper include computational experiments? [yes]
\begin{itemize}
	% GS: are you sure you don't want to append the code? I think it makes a better impression (that we really did the thing :)) and no one is going to check it in too much detail anyway...
    % DC: I'm not sure what other reviewers think but I never cared if people attached code or not because I always saw it as the authors' loss for not attaching code for various reasons. I just don't want to do more work:) and have people steal code when the work hasn't been accepted yet
    \item Any code required for pre-processing data is included in the appendix. [no] 
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. [no] 
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. [yes]
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from [yes]
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. [yes] 
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. [partial]
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. [yes]
    \item This paper states the number of algorithm runs used to compute each reported result. [yes]
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. [yes]
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). [no] 
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper's experiments. [yes]
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. [yes]
\end{itemize}


==> tables/coverage.tex <==
% \begin{tabularx}{\columnwidth}{X Y Y Y}
%     \toprule
%     Domain      & \lama & \baseline & \lrnn \\
%     \midrule
%     Blocksworld & 54    & 60        & 60    \\
%     Ferry       & 60    & 60        & 60    \\
%     Rovers      & 60    & 60        & 60    \\
%     Satellite   & 56    & 60        & 60    \\
%     \bottomrule
% \end{tabularx}

\begin{tabularx}{\columnwidth}{X Y Y Y Y}
    \toprule
    Planner      & Blocks & Ferry & Rover & Satellite \\
    \midrule
    \baseline & 60 & 60 & 60 & 60 \\
    \lama & 54 & 60 & 56 & 60 \\
    \lrnn & 60 & 60 & 58 & 60 \\
    \bottomrule
\end{tabularx}

